Semi-supervised Anomaly Detection with Extremely Limited Labels in Dynamic Graphs

Semi-supervised graph anomaly detection (GAD) has recently received increasing attention, which aims to distinguish anomalous patterns from graphs under the guidance of a moderate amount of labeled data and a large volume of unlabeled data. Although these proposed semi-supervised GAD methods have achieved great success, their superior performance will be seriously degraded when the provided labels are extremely limited due to some unpredictable factors. Besides, the existing methods primarily focus on anomaly detection in static graphs, and little effort was paid to consider the continuous evolution characteristic of graphs over time (dynamic graphs). To address these challenges, we propose a novel GAD framework (EL$^{2}$-DGAD) to tackle anomaly detection problem in dynamic graphs with extremely limited labels. Specifically, a transformer-based graph encoder model is designed to more effectively preserve evolving graph structures beyond the local neighborhood. Then, we incorporate an ego-context hypersphere classification loss to classify temporal interactions according to their structure and temporal neighborhoods while ensuring the normal samples are mapped compactly against anomalous data. Finally, the above loss is further augmented with an ego-context contrasting module which utilizes unlabeled data to enhance model generalization. Extensive experiments on four datasets and three label rates demonstrate the effectiveness of the proposed method in comparison to the existing GAD methods.

==> subtexes/conclusion_short.tex <==
In this paper, we make the first attempt to tackle the anomaly detection problem in dynamic graphs under the challenging condition of extremely limited labels. Our proposed EL$^{2}$-DGAD framework introduces a transformer-based graph encoder to capture the evolving graph patterns from both local and global perspectives. This is further augmented with an ego-context hypersphere classification loss and contrastive loss, designed to effectively harness limited labels and abundant unlabeled data. Extensive experiments across various datasets and label rates demonstrate its superiority over existing GAD methods.

==> subtexes/experiment_short.tex <==
%\section{Experiments}

%\subsection{Experimental Setup}

\subsection{Experimental Settings}
\subsubsection{Datasets and Model Implementation}

% In this paper, we adopt three real-world datasets: Wikipedia~\cite{kumar2019predicting}, UCI~\cite{opsahl2009clustering}, and Digg~\cite{de2009social}. Following~\cite{taddy}, we inject $3\%$ of artificial anomalous edges into UCI and Digg which do not have anomalies. These datasets are chronologically split into training, validation, and testing by the ratio 50/20/30 based on interaction timings. In this paper, We specifically test under extremely limited label conditions with only 1, 2, or 3 anomaly labels, proportionally masking normal labels to maintain a consistent anomaly ratio. 

We evaluate our approach on four dynamic network datasets: UCI, Digg, Reddit, and Wikipedia~\cite{opsahl2009clustering, de2009social, kumar2019predicting}. 
Since UCI and Digg lack labeled anomalies, we
inject 3$\%$ synthetic anomalies similar to~\cite{taddy}. All datasets are chronologically split into training (50\%), validation (20\%), and testing (30\%) to reflect real-world scenarios where future data is unknown during training. We evaluate performance under extremely limited labels, providing only 1, 2, or 3 labeled anomaly examples, with labeled normal samples retained proportionally. 

To construct the ego-graph $\mathcal{G}^t$, we retain all edges up to and including time $t$. The context graph $\mathcal{G}^{t^{-}}$ similarly includes edges up to $t$ but excludes those occurring exactly at $t$, ensuring it represents only historical information. To manage the potentially large sizes of $\mathcal{G}^t$ and $\mathcal{G}^{t^{-}}$, we sample 25, 10, and 5 neighboring nodes at the first, second, and third hops, respectively, while ensuring sampled events occur before the target edge’s timestamp.
In addition, our model uses a two-layer transformer with 4 attention heads, and the hidden size is set to 128 across all modules. The contrastive loss weight $\lambda$ is set to 0.01 for Digg, UCI, Reddit and 10 for Wikipedia. The models are trained for 20 epochs using the Adam optimizer~\cite{kingma2014adam}, with a learning rate of 0.0001 for the Digg and UCI datasets, and 0.001 for the Wikipedia and Reddit dataset.

\subsubsection{Baselines and Performance Evaluation}

We benchmark our proposed method against several recent GAD models, namely GDN~\cite{ding2021few}, SL-GAD~\cite{zheng2021generative}, PREM~\cite{pan2023prem}, AddGraph~\cite{zheng2019addgraph}, TADDY~\cite{taddy}, TGAT~\cite{tgat}, and SAD~\cite{tian2023sad}. Among these, GDN, SL-GAD, and PREM are designed for static graph anomaly detection, while AddGraph, TADDY, TGAT, and SAD are tailored for dynamic graph settings. Note that only GDN, TADDY, AddGraph, and SAD can utilize label information by design. For a fair, label-inclusive comparison for other models, we perform a similar setting as in~\cite{tian2023sad}: applying a cross-entropy loss to the edge representations, which are derived from the concatenated node embeddings of the edge endpoints. Thus, the performance of all models can be evaluated based on the classification results.  

\subsection{Comparison with State-of-the-art GAD}

Extensive results in Table~\ref{tab: comparison_results} show that EL$^{2}$-DGAD consistently outperforms all baselines across four datasets, especially under extremely limited labeled anomalies. The decline in performance for GDN, PREM, and SL-GAD validates our hypothesis regarding the critical role of dynamic information. 
% Although AddGraph and TADDY are designed for dynamic graphs, they rely on discrete snapshots which are at the risk of losing fine-grained temporal details. Moreover, they lack a robust semi-supervised learning mechanism, making it challenging to effectively utilize the limited labeled data. 
The underperformance of AddGraph and TADDY is likely due to their use of discrete graph snapshots and the lack of a robust semi-supervised loss, which is essential when labels are scarce.
Despite SAD being a recent advanced semi-supervised AD approach for dynamic graphs, it also shows a decline in performance under severe label scarcity.
% In contrast, our method operates directly on continuous dynamic graphs, with a transformer-based encoder that attends to the most relevant neighbors using fine-grained temporal information. Additionally, our ego-context hypersphere classification loss aligns each edge with its surrounding temporal and structural context, enabling EL$^{2}$-DGAD to better detect anomalies that deviate from normal patterns.
Specifically, SAD relies on a deviation network to generate pseudo-labels, which weakens the contrastive learning component when only a few labeled examples are available. In contrast, our method decouples supervised and unsupervised learning, allowing effective generalization with minimal labels. Moreover, our approach offers two key advantages. First, our ego-context hypersphere loss delivers a more precise instance-wise comparison than the deviation network, which relies on global statistics. Second, our model employs a more robust transformer-based encoder in comparison to the GAT encoder in SAD, which additionally improves dynamic graph learning from a global perspective.

% Extensive results in Table~\ref{tab: comparison_results} show that our EL$^{2}$-DGAD consistently surpasses all comparison methods across four datasets, particularly when label availability is low. The decline in performance for GDN, PREM, and SL-GAD validates our hypothesis regarding the critical role of dynamic information. The underperformance of AddGraph and TADDY is likely due to their use of discrete graph snapshots and the lack of a robust semi-supervised loss, which is essential when labels are scarce. Despite SAD being a recent advanced semi-supervised AD approach for dynamic graphs, it also shows a decline in performance under severe label scarcity. This drop is likely tied to its use of pseudo-labels derived from deviation scores, which become less reliable when labels are extremely scarce. Overall, the improvement of our model gains stems from efficiently utilizing limited labels through two specialized losses and a graph encoder that adeptly captures dynamic local and global interactions.

\begin{table*}[t]
\caption{Performance comparison for all methods in terms of AUC.}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \hline
     Dataset & \multicolumn{3}{c|}{Wikipedia} & \multicolumn{3}{c|}{UCI} & \multicolumn{3}{c|}{Digg} & \multicolumn{3}{c}{Reddit} \\
    \cline{1-13}
     Labels & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3 \\
    \hline


    AddGraph & 0.631 & 0.641 & 0.663 & 0.732 & 0.732 & 0.754 & 0.739  & 0.740 & 0.742 & 0.578 & 0.580 & 0.582\\TGAT & 0.660 & 0.674 & 0.694 & 0.764 & 0.790 & 0.808 & 0.800 & 0.804 & 0.812 & 0.527 & 0.541 & 0.555 \\GDN & 0.516 & 0.529 & 0.533 & 0.510 & 0.546 & 0.547 & 0.511 & 0.510 & 0.513 & 0.532 & 0.531 & 0.533 \\SL-GAD & 0.467 & 0.524 & 0.526 & 0.503 & 0.497 & 0.502 & 0.494 & 0.497 & 0.504 & 0.503  &0.505  &0.500  \\TADDY & 0.616 & 0.617 & 0.618 & 0.769 & 0.765 & 0.772 & 0.811 & 0.841 & 0.842 & 0.516  &0.517  & 0.518 \\
    SAD & 0.661 & 0.674 & 0.710 & 0.774 & 0.798 & 0.816 & 0.809 & 0.820 & 0.841 & 0.561  & 0.566 & 0.592
    \\PREM & 0.549 & 0.555 & 0.555 & 0.531 & 0.532 & 0.536 & 0.512 & 0.513 & 0.515  & 0.516 & 0.535 & 0.536\\ \hline 
    EL$^2$-DGAD & \textcolor{blue}{\textbf{0.722}} & \textcolor{blue}{\textbf{0.725}} & \textcolor{blue}{\textbf{0.732}} & \textcolor{blue}{\textbf{0.839}} & \textcolor{blue}{\textbf{0.840}} & \textcolor{blue}{\textbf{0.842}} & \textcolor{blue}{\textbf{0.839}} & \textcolor{blue}{\textbf{0.844}} & \textcolor{blue}{\textbf{0.846}} & \textcolor{blue}{\textbf{0.611}} & \textcolor{blue}{\textbf{0.615}} & \textcolor{blue}{\textbf{0.616}} \\

  \hline
  \end{tabular}}
  \label{tab: comparison_results}
\end{table*}



\subsection{Ablation Experiments}

% Table~\ref{tab:ablation_results} reports the outcomes of the ablation experiment. In general, EL$^{2}$-DGAD achieves optimal results with all components intact. The removal of local MHA significantly impairs performance due to its vital role in capturing neighborhood structure. Conversely, omitting global MHA has also a noticeable negative impact, which reinforces the necessity of capturing node interactions from a global perspective. Additionally, our model outperforms the ``Local+Global MHA'', where local and global MHA are performed independently and their outputs simply added. This demonstrates the effectiveness of our way of integrating them sequentially. 
% Moreover, removing the integration of fine-grained timestamp information from the attention mechanism in the Transformer significantly degrades the performance, this shows the importance of modeling the temporal dynamics in the graph, which can be crucial to capture time-sensitive anomalies.
% Furthermore, the decrease in performance without the contrastive loss component confirms the importance of mining the unlabeled data. Finally, removing ego-context contrasting from $L^{echsc}$ (resort to Eq.~\ref{eq. hsc}), results in a notable performance drop, which emphasizes the importance of explicitly using dynamic neighbor information to assist classification.


Table~\ref{tab:ablation_results} presents the results of the ablation study. Overall, EL$^{2}$-DGAD achieves optimal performance when all components are included. Specifically, removing the local MHA or global MHA significantly degrades performance, underscoring the importance of capturing both neighborhood structures and global interactions.
Omitting fine-grained timestamp integration also leads to a considerable drop, as it hinders the model from capturing essential temporal dynamics. Additionally, the drop in performance without the contrastive loss component $\mathcal{L}^{ecc}$ indicates the value of leveraging unlabeled data to improve anomaly detection accuracy. Finally, eliminating the ego-context contrast from $\mathcal{L}^{echsc}$ forces all normal instances toward a single center, limiting the model's ability to capture diverse normal behaviors and effectively distinguish anomalies.



\begin{table}[t]
\caption{Performance evaluation on ablation experiments in terms of AUC.}
  \centering
  %\resizebox{1\linewidth}{!}{
  \begin{tabular}{c|ccc|ccc|ccc}
    \hline
    Dataset & \multicolumn{3}{c|}{Wikipedia} & \multicolumn{3}{c|}{UCI}  & \multicolumn{3}{c}{Digg} \\ \cline{1-10}
    
     Labels & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3  \\
     
    \hline
    $w/o$ Local MHA & 0.563 & 0.569 & 0.582 & 0.771 & 0.775 & 0.772 & 0.808 & 0.796 & 0.802 \\
    $w/o$ Global MHA & 0.694 & 0.709 & 0.716 & 0.835 & 0.836 & 0.838 & 0.802 & 0.807 & 0.800 \\
    % Local+Global MHA & 0.695 & 0.708 & 0.708 & 0.835 & 0.842 & 0.845 & 0.814 & 0.819 & 0.825 \\
    $w/o \ \phi(t)$ in MHA & 0.465 & 0.473 & 0.474 & 0.789 & 0.791 & 0.800 & 0.719 & 0.730 & 0.756 \\
    $w/o$ $\LL^{ecc}$ & 0.653 & 0.683 & 0.683 & 0.838 & 0.837 & 0.840 & 0.815 & 0.821 & 0.821 \\
    $w/o$ ego-context in $\LL^{echsc}$ & 0.650 & 0.683 & 0.704 & 0.824 & 0.824 & 0.837 & 0.730 & 0.745 & 0.745 \\ \hline
    EL$^{2}$-DGAD &  \textcolor{blue}{\textbf{0.722}} &  \textcolor{blue}{\textbf{0.725}} &  \textcolor{blue}{\textbf{0.732}} &  \textcolor{blue}{\textbf{0.839}} & \textcolor{blue}{\textbf{0.840}}& \textcolor{blue}{\textbf{0.842}}& \textcolor{blue}{\textbf{0.839}}& \textcolor{blue}{\textbf{0.844}}& \textcolor{blue}{\textbf{0.846}} \\ \hline
  \end{tabular}%}
\label{tab:ablation_results}
\end{table}


% \subsection{Parameters Sensitivity}

% Figure~\ref{fig: sensitivity_results} illustrates the AUC performance for three datasets (Digg, UCI, and Wikipedia) as it varies with changes in the balance parameter $\lambda$ for the ego-context contrastive learning component and the number of neighbors in the first hop. In Figure 2(a), the Wikipedia dataset shows improved AUC scores with higher $\lambda$ values compared to Digg and UCI. This may be due to the greater complexity of anomalies in Wikipedia, making it a more challenging task under extremely limited conditions. Consequently, increasing $\lambda$ enhances the model’s ability to capture general patterns of normal samples, which improves the robustness of the model. 
% \begin{figure}[t]
% \begin{subfigure}[b]{1\linewidth}
%     \centering
%     \includegraphics[height=0.7cm]{figures/legend.eps}
%     %\caption{AUC vs. balance parameter $\lambda$}
%     % \label{fig: contra_results}
% \end{subfigure}
% \newline
% \begin{subfigure}[b]{0.49\linewidth}
%     \centering
%     \includegraphics[height=3.2cm]{figures/contra_results.eps}
%     \caption{AUC vs. balance parameter $\lambda$}
%      \label{fig: contra_results}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.49\linewidth}
%     \centering
%     \includegraphics[height=3.2cm]{figures/neighbor_results.eps} 
%     \caption{AUC vs. number of neighbors}
%     \label{fig: neighbor_results}
% \end{subfigure}
% \caption{Sensitivity analysis of $\lambda$ and neighbors number when there is one labeled anomaly available in the training dataset.}
% \label{fig: sensitivity_results}
% \end{figure}

% In Figure 2(b), AUC performance for all three datasets slightly increases as the number of neighbors rises, indicating that additional neighborhood information helps the model better distinguish between normal and anomalous interactions within the graphs. Overall, the model’s sensitivity to changes in $\lambda$ and the number of neighbors remains relatively low, suggesting that it is robust to variations in these hyperparameters.


\subsection{t-SNE Visualization} 

Figure~\ref{fig: visualization} shows t-SNE visualizations of the output embeddings from the layer before anomaly scoring in the Wikipedia dataset, where the selected three models were trained with supervision from only one labeled anomaly. 
% In the embeddings produced by AddGraph, anomalies are dispersed throughout the normal samples, indicating a limited capacity for distinguishing between normal and anomalous instances. Similarly, SAD shows slight improvement with a relatively better separation, but anomalies remain scattered and intermingled within the normal clusters, lacking a clear boundary. In contrast, 
Our proposed EL$^{2}$-DGAD exhibits a relatively clearer separation, with anomalies forming distinct clusters that are well-separated from normal samples. This distinct clustering suggests that EL$^{2}$-DGAD more effectively learns discriminative embeddings, allowing it to capture the subtle distinctions between normal and anomalous interactions. 

\begin{figure}[t]
\begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[height=2.6cm]{figures/TSNE_AddGraph_wikipedia_124_1_124.eps}
    \caption{AddGraph}
     \label{fig: addgraph_tsne}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[height=2.6cm]{figures/TSNE_SAD_wikipedia_1_1_123.eps}
    \caption{SAD}
    \label{fig: sad_tsne}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\linewidth}
    \centering
    \includegraphics[height=2.6cm]{figures/TSNE_ours_wikipedia_7_1_123.eps}
    \caption{EL$^{2}$-DGAD (ours)}
     \label{fig: ours_tsne}
\end{subfigure}
\caption{t-SNE Visualization on the Wikipedia dataset.}
\label{fig: visualization}
\end{figure}







==> subtexes/introduction.tex <==
Anomaly detection (AD) is the process of identifying irregular patterns in data that deviate from expected behavior~\cite{chandola2009anomaly}. In today's interconnected world, many datasets from various domains inherently form complex network structures~\cite{wei2021branch,yang2020tensor,yang2019survey,chen2022antibenford,tang2008arnetminer}. These network structures are often contaminated with anomalies. For instance, financial networks may exhibit irregular transactional patterns indicative of fraud, while social networks could contain spurious accounts engaged in malicious activities. In light of the inherent complexity of these graph-structured datasets and the severe consequences of ignoring anomalies, there has been a growing research emphasis on graph anomaly detection (GAD) in recent years.

% Existing GAD methods predominantly rely on either unsupervised or semi-supervised learning techniques. Unsupervised GAD methods typically utilize reconstruction-based~\cite{ding2019deep,luo2022comga,zhang2022unsupervised} or contrastive learning-based tasks~\cite{liu2021anomaly,zheng2021generative,zhang2022reconstruction,pan2023prem}, to learn normal patterns in unlabeled data. Anomalies are then detected as deviations from these patterns. For instance, DOMINANT~\cite{ding2019deep} utilizes an auto-encoder architecture to reconstruct graph structures and attributes, under the premise that anomalies will result in noticeable reconstruction errors. COLA~\cite{liu2021anomaly} applies contrastive learning by comparing nodes to their respective subgraphs. Anomalies are thus identified based on inconsistencies highlighted by contrastive loss. 
% Similarly, PREM~\cite{pan2023prem} uses a propagation matrix to extract ego and neighbor features, which are encoded through MLPs and optimized with contrastive learning, identifying anomalies based on the cosine similarity between the embeddings.

Existing GAD methods primarily utilize either unsupervised or semi-supervised learning approaches. In unsupervised GAD, reconstruction-based~\cite{ding2019deep,luo2022comga,zhang2022unsupervised} and contrastive learning-based techniques~\cite{liu2021anomaly,zheng2021generative,zhang2022reconstruction,pan2023prem} are widely adopted to model normal patterns in unlabeled data. Anomalies are then detected as deviations from these patterns. For example, reconstruction-based methods like DOMINANT~\cite{ding2019deep} and ComGA~\cite{luo2022comga} employ autoencoders to reconstruct graph structures and attributes, whereas anomalies are identified through significant reconstruction errors. On the other hand, contrastive learning-based methods, such as COLA~\cite{liu2021anomaly} and PREM~\cite{pan2023prem}, detect anomalies by learning to differentiate normal patterns. COLA compares nodes with their subgraphs to expose inconsistencies via contrastive loss, while PREM evaluates the similarity between ego and neighbor embeddings to assign anomaly scores.

However, unsupervised learning in AD may risk identifying noisy samples as anomalies due to the lack of prior anomaly knowledge. In practical scenarios, it is often possible to acquire a limited set of labeled examples. This has spurred increased attention towards semi-supervised GAD, which combines labeled data with unlabeled data to improve detection performance~\cite{wang2019semi,kumagai2021semi,meng2021semi,ding2021few,tian2023sad}. For example, SemiADC~\cite{meng2021semi} employs generative adversarial networks to learn the feature distribution of normal nodes from unlabeled data and then uses a binary classifier to differentiate these generated normal features from the labeled abnormal ones. GDN~\cite{gdn} adopts a deviation loss to enforce significant differences between the anomaly scores of normal and abnormal nodes, using a reference score derived from labeled anomalies and unlabeled data to guide the learning process. Similarly, SAD~\cite{tian2023sad} uses a memory-enhanced deviation network to enforce significant deviations between abnormal and normal nodes, and incorporates a contrastive learning module to harness the potential of unlabeled data.

Despite the promising results of semi-supervised GAD, challenges still exist. A primary issue is its inherent assumption that a sufficient number of labels, particularly for anomalies, are readily available. However, the rarity and difficulty in accurately identifying anomalies make this assumption impractical in real-world applications, consequently hampering the effectiveness of GAD methods. Additionally, most existing GAD methods are designed for static graphs, failing to consider the dynamic nature of real-world graphs that are characterized by constantly evolving nodes, edges, and attributes. Dynamic information can sometimes play a crucial role in identifying anomalies. For instance, a sudden spike in account creation during off-peak hours in social networks could indicate inauthentic behavior, while unexpected large transfers during typically low-transaction periods in financial networks may signal irregular activity.


To address these challenges, we propose EL$^{2}$-DGAD, a novel GAD method designed to bolster the robustness of existing methods in handling dynamic graphs under the constraints of extremely limited labeling. Specifically, a transformer-based graph encoder is introduced to our EL$^{2}$-DGAD, which aims to capture both local and global perspectives of the graph. This is achieved through a combination of local and global attention mechanisms, departing from traditional message-passing mechanisms that fall short of capturing the global context of graphs~\cite{xu2018how,morris2019weisfeiler}. We further integrate the continuous-time dynamics into the attention, preserving detailed temporal information in contrast to methods that rely on discrete graph snapshots~\cite{zheng2019addgraph,liu2021anomaly,cai2021structural}. To effectively utilize the limited labels, we adopt an ego-context hypersphere classification loss. It promotes compact representations of normal instances based on dynamic context while refining classification boundaries using limited anomalies. To further improve model generalization, we integrate an ego-context contrastive loss that aligns the neighboring information to target instances from the vast amount of unlabeled data. 

To summarize, our main contributions include:

\begin{itemize}
\item To the best of our knowledge, we are the first attempt to investigate and address anomaly detection problem in dynamic graphs with extremely scarce labeling.
    
\item We propose a simple and effective GAD framework designed to enhance the generalization of existing GAD methods in scenarios with limited labeling for dynamic graphs. A transformer-based graph encoder is first proposed to model dynamic graphs from both local and global perspectives. Furthermore, an ego-context hypersphere classification loss and contrastive loss are incorporated, specifically designed to effectively utilize limited labels, mitigate overfitting and enhance model generalization.

\item Extensive experiments on three datasets and three extremely low label rates demonstrate the effectiveness of the proposed method in comparison to existing GAD methods.
\end{itemize}

==> subtexes/introduction_short.tex <==
Anomaly detection identifies irregular patterns in data that deviate from expected behavior~\cite{chandola2009anomaly}. In today's interconnected world, many datasets naturally form complex network structures that are often contaminated with anomalies, such as fraudulent transactions in financial networks or malicious accounts in social networks~\cite{wei2021branch,chen2022antibenford}. Given the inherent complexity of these graph-structured datasets and the severe consequences of ignoring anomalies, graph anomaly detection (GAD) has garnered significant attention in recent years.

Owning to the rarity of anomalies, existing GAD methods mainly rely on unsupervised approaches, including reconstruction-based~\cite{ding2019deep,luo2022comga,zhang2022unsupervised} and contrastive learning-based techniques~\cite{liu2021anomaly,zheng2021generative,pan2023prem}. These methods detect anomalies as deviations from learned normal patterns but mostly focus on static graphs, overlooking the dynamic evolution of nodes, edges, and attributes. Recently, dynamic GAD has received increasing research interest, which requires models capable of capturing both structural dependencies and temporal patterns~\cite{zheng2019addgraph}. While some methods model dynamic graphs as discrete snapshots using techniques such as GCNs, GRUs, or transformers~\cite{zheng2019addgraph,cai2021structural,taddy}, they are primarily unsupervised and rely heavily on the quality of the pseudo labels, which may risk identifying noisy samples as anomalies due to the lack of prior anomaly knowledge. 

% Owing to the rarity of anomalies in real-world applications, existing GAD methods primarily rely on unsupervised approaches such as reconstruction-based ~\cite{ding2019deep,luo2022comga,zhang2022unsupervised} or contrastive learning-based techniques~\cite{liu2021anomaly,zheng2021generative,pan2023prem}. Reconstruction-based techniques (e.g., DOMINANT~\cite{ding2019deep} and ComGA~\cite{luo2022comga}) employ autoencoders to reconstruct graph structures and attributes, whereas anomalies are identified through substantial reconstruction errors. Whereas contrastive learning-based methods (e.g., COLA~\cite{liu2021anomaly} and PREM~\cite{pan2023prem}) detect anomalies by comparing nodes with their surrounding structures and identifying anomalies that have large inconsistencies highlighted via contrastive losses. However, these methods primarily target static graphs, neglecting the dynamic evolution of nodes, edges, and attributes in real-world networks.

% Recently, detecting anomalies in dynamic graphs has received increasing research interest, which requires models capable of capturing both structural dependencies and temporal patterns~\cite{zheng2019addgraph,cai2021structural,taddy}. For example, 
% AddGraph\cite{zheng2019addgraph} models dynamic graphs as sequential snapshots using GCNs~\cite{kipf2017semi} and GRUs~\cite{chung2014empirical}, and employ a margin-based loss to distinguish normal edges from pseudo-anomalous edges generated through selective negative sampling. Similarly, TADDY~\cite{taddy} employs a transformer on discrete snapshots to capture static and temporal patterns, and uses a binary classifier to distinguish anomalies from pseudo-anomalous edges. However, these methods are primarily unsupervised and rely heavily on the quality of the pseudo labels, which may risk identifying noisy samples as anomalies due to the lack of prior anomaly knowledge. 

In practice, it is often possible to acquire a limited set of labeled examples. This has spurred increased attention towards semi-supervised GAD, which combines labeled data with unlabeled data to improve detection performance~\cite{kumagai2021semi, meng2021semi, ding2021few, tian2023sad,chen2024towards}. For instance, SemiADC~\cite{meng2021semi} uses generative adversarial networks to learn the feature distribution of normal nodes and trains a classifier to distinguish them from labeled anomalies. Similarly, 
SAD~\cite{tian2023sad} uses a memory-enhanced deviation network to enforce significant deviations between abnormal and normal nodes, and incorporates a contrastive learning module to harness the potential of unlabeled data.
Despite their promising results, these methods rely heavily on labeled anomalies, which are scarce and difficult to obtain, thus limiting their practical effectiveness in real-world applications. 


To our knowledge, no prior work has explored dynamic GAD under severely limited supervision, where only a handful of labeled anomalies are available during training. To bridge this gap, we present the first investigation into this problem and propose a novel framework, EL$^{2}$-DGAD, which enhances the robustness of existing GAD methods in dynamic settings with minimal supervision.
First, a transformer-based dynamic graph encoder is introduced to effectively capture both temporal and structural properties of dynamic graphs. Unlike existing methods that primarily focus on local dependencies using GNN-based approaches~\cite{tgat,tian2023sad}, our encoder leverages both local and global attention mechanisms. The former extracts fine-grained patterns from a node's neighborhood, while the latter aggregates these patterns across the graph, thereby enhancing the detection of subtle and extensive anomalies across the graph. 
Additionally, continuous-time embeddings are integrated into the transformer's attention mechanism, enabling precise, time-sensitive representations. This contrasts with discrete snapshot-based methods~\cite{zheng2019addgraph,liu2021anomaly,cai2021structural}, which lose precision by grouping events into fixed intervals, making it harder to detect time-sensitive anomalies.
To effectively utilize the limited labels, we propose an ego-context hypersphere classification loss, which learns a context-aware hypersphere boundary by considering both the ego (target instance) and its historical context (graph dynamics). Rather than modeling the diverse and irregular nature of anomalies, it establishes a robust boundary for normal data, reducing reliance on a large number of labeled anomalies. 
Lastly, to further improve model generalization, we integrate an ego-context contrastive loss, which ensures the consistency of neighboring information with target instances by utilizing the vast amount of unlabeled data. Extensive experiments on four datasets and three extremely low label rates demonstrate the effectiveness of the proposed method in comparison to existing GAD methods.


% To summarize, our main contributions include:

% \begin{itemize}

% \item To the best of our knowledge, we are the first to investigate and address anomaly detection in dynamic graphs with extremely scarce labeling.
% \item We propose a transformer-based dynamic graph encoder aiming to capture local and global structural dependencies while integrating continuous-time dynamics, enhancing the detection of subtle and time-sensitive anomalies.
% \item We introduce an ego-context hypersphere classification loss to establish a robust context-aware boundary for normal patterns and an ego-context contrastive loss to leverage unlabeled data, enabling effective anomaly detection under minimal supervision.
% \item Extensive experiments on four datasets and three extremely low label rates demonstrate the effectiveness of the proposed method in comparison to existing GAD methods.

% \end{itemize}







==> subtexes/methodology_short.tex <==
\subsection{Problem Formulation}

% In this paper, a dynamic graph is defined as $\G=(\V,\E)$, where $\V$ represents different nodes, $\E$ comprises temporal edges and each edge is denoted as $\delta^t=(v_i, v_j, t, {x}_{ij})$. This tuple signifies an interaction from node $v_i$ to $v_j$ at time $t$, enriched with edge feature $x_{ij}$. Additionally, We define $\G^t$ as the subgraph containing all events up to time $t$, and $\G^{t^{-}}$ as the same, excluding the event at $t$.

% Our proposed EL$^{2}$-DGAD aims to identify anomalous edges, with each edge $\delta^t$ potentially having a latent label $y^t$ with 0 as normal and 1 as abnormal. In this study, we have access to only a limited subset of labels, denoted by $Y^L$, with the remainder being unlabeled, represented as $Y^U$, and $|Y^L|\ll|Y^U|$. We aim to develop an algorithm assigning anomaly scores to each edge, i.e., $f(\delta^t)=s^t$, effectively differentiating between normal and anomalous edges.

In this paper, we define a dynamic graph as $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ represents the set of nodes and $\mathcal{E}$ consists of temporal edges. Each edge, denoted by $\delta^t = (v_i, v_j, t, x_{ij})$, captures an interaction from node $v_i$ to node $v_j$ at time $t$, with $x_{ij}$ serving as the edge feature. 
Additionally, We define $\mathcal{G}^t$ as the subgraph containing all events up to time $t$, and $\mathcal{G}^{t^{-}}$ as the same, excluding the event at $t$.
Our proposed EL$^{2}$-DGAD framework aims to detect anomalous edges in this dynamic graph setting, where each edge $\delta^t$ is associated with a latent label $y^t$, indicating whether the edge is normal ($y^t = 0$) or abnormal ($y^t = 1$). In this study, we have access to only a limited number of labeled edges, denoted as $Y^L$, while the majority of edges remain unlabeled ($Y^U$), with $|Y^L| \ll |Y^U|$. The goal is to develop an algorithm that assigns an anomaly score $s^t$ to each edge, represented as $f(\delta^t) = s^t$, to effectively distinguish between normal and anomalous edges.

\subsection{Overview}

The overview of EL$^{2}$-DGAD is shown in Figure~\ref{fig: EL2DGAD_framework}. Specifically, for each input sample, an ego and a context graph are simultaneously defined. Each of the graphs is encoded through a transformer-based dynamic graph encoder, which builts on top of a series of local and global attentions (Section~\ref{sec: graph_encoder}). During model training, we introduce an ego-context hypersphere classification loss in Section~\ref{sec: semi-supervised loss} that classifies edges by quantifying the similarity between their ego representation and the corresponding dynamic neighboring context. Finally, an ego-context contrastive loss in Section~\ref{sec: contrastive loss} is incorporated that is designed to mine and learn from the patterns of normality prevalent within the graph based on unlabeled data.
\begin{figure*}[t]
    \centering
    \includesvg[width=\linewidth]{figures/architecture_large_flat.svg}
    %\includegraphics[width=\linewidth]{figures/architecture_large.eps}
    % \caption{The architecture of EL$^{2}$-DGAD. The bottom section shows the ego and context graphs for two example edges (one normal and one abnormal), processed by the graph encoder in the top section. For a given edge, the distance between encoded ego and context graphs is minimized if the edge is normal and maximized if it is abnormal (via $\mathcal{L}^{ecc}$). Additionally, $\mathcal{L}^{echsc}$ regularizes all edges, enforcing consistency between each edge’s representation and its context graph. For the graph encoder, each layer includes a local MHA module that aggregates information from neighboring edges and nodes, along with the time difference relative to the edge’s timestamp. The local MHA outputs are then fed into a global MHA, followed by feed-forward networks and layer normalization.}
    \caption{An illustration for the architecture of EL$^{2}$-DGAD.}
    \label{fig: EL2DGAD_framework}
\end{figure*}

\subsection{Graph Encoder}
\label{sec: graph_encoder}

In scenarios with extremely limited labeled data, a robust model must capture both temporal and structural dependencies in dynamic graphs. Inspired by recent graph transformer advances~\cite{ying2021transformers,chen2022structure}, We propose a transformer-based dynamic graph encoder that leverages local attention for fine-grained neighborhood extraction, global attention for graph-wide aggregation, and continuous-time embeddings to seamlessly capture temporal dynamics. Concretely, our graph encoder takes a subgraph at time $t$ as the input (e.g., $\G^{t}$ or $\G^{t^{-}}$) and generates node representations that reflect their dynamic state. We start by aggregating 1-hop neighborhood information through masked multi-head self-attention (local MHA). To capture the evolving nature of dynamic graphs, we define the entries of $Q$, $K$, and $V$ at layer $l$ as follows:
\begin{align}
Q^l_{ij} = \text{MLP}(\text{Concat}(x_{ij}, z^{l-1}_i, z^{l-1}_j, \phi(\Delta_t)))W^{Q,l} \\
K^l_{ij} = \text{MLP}(\text{Concat}(x_{ij}, z^{l-1}_i, z^{l-1}_j, \phi(\Delta_t)))W^{K,l} \\
V^l_{ij} = \text{MLP}(\text{Concat}(x_{ij}, z^{l-1}_i, z^{l-1}_j, \phi(\Delta_t)))W^{V,l}
\end{align}
where $z^{l-1}_i$ is the output for node $i$ from layer $l-1$, and $z_i^0$ is a learnable embedding vectors specified by the degree of $v_i$, as detailed in~\cite{ying2021transformers}. MLP denotes the multi-layer perceptrons. $\Delta_t=t-t_{ij}$, where $t_{ij}$ is the occurring time of edge $(v_i, v_j)$. $\phi(\cdot)$ is the sinusoidal embedding function~\cite{transformer}, which generates a time representation by applying sine and cosine functions to the input time difference $\Delta_t$, scaled by a range of frequencies. 

Then, the attention output of node $i$ for a single head can be formulated as:
\begin{align}
    a^l_i= \sum_{j}\text{softmax}_j\left(\frac{Q^l_{ij}{K^l}^T_{ij}}{\sqrt{d}} M_{ij} \right)V^l_{ij}
\end{align}
where $M$ is the adjacency matrix of the input graph. Next, we fed the outputs obtained from the local MHA, as the input to the regular multi-head self-attention in~\cite{transformer} (global MHA). 
% Local MHA focuses on learning neighborhood information which is similar to GNNs but with their inherent limitations, whereas global attention broadens the perspective without explicit structural reliance. Thus, this combination enhances the expressiveness of our model in representing graph structures, effectively balancing the strengths of local and global information processing. 
The layer $l$'s output is then defined as
\begin{align}
    z^l=\text{LN}(\text{FFN}(z^{l-1, loc}+z^{l-1,glo}))+z^{l-1, loc}+z^{l-1, glo}
\end{align}
where $z^{l-1, loc}$ and $z^{l-1, glo}$ are the output from the local MHA and global MHA, LN and FFN denote the layer normalization and the feed-forward blocks.



\subsection{Model Training}

\subsubsection{Ego-context HSC loss} 
\label{sec: semi-supervised loss}

To train the model, we incorporate the hypersphere classification (HSC) loss~\cite{ruff2020rethinking}, which is well-suited for anomaly detection tasks when labeled anomalies are scarce.  Traditional classifiers assume similar data points cluster naturally, but anomalies rarely form distinct clusters~\cite{chandola2009anomaly}. The HSC loss overcomes this by constructing a spherical decision boundary that pulls normal samples toward a fixed center (the zero vector) and pushes anomalies away. Specifically, the HSC loss of a given sample at $t$ is defined as:
\begin{align}
% L = y_t\|\phi(\delta(t))\|^2 + (1-y_t)\log(1-\exp{(-\|\phi(\delta_t)\|^2)})
\LL_t^{hsc} = -y^t \log{l(x^t)} - (1-y^t) \log{(1-l(x^t))}
\label{eq. hsc}
\end{align}
where $l(z)=\exp{(-\|z\|^2)}$, $x^t$ and $y^t$ are the latent representation and label of an interaction event at time $t$. The final classification output is given by $1-l(x^t)$, which represents the probability of an interaction being classified as normal.
% This formulation is a variant of the cross-entropy loss but with a unique focus: it constructs a spherical decision boundary that compacts normal samples towards a fixed center (the zero vector), while pushing anomalies away by maximizing their distance from this center. In essence, the goal is to pull normal data points closer to the origin, creating a compact representation, and to push out anomalous points to better distinguish them. 

To capture the dynamic nature of graphs, we modify the HSC loss to incorporate temporal and structural context. Specifically, we represent the interaction at time $t$ using two graph perspectives: the ego graph $\G^t$, which captures the evolving interactions including the event at $t$, and the context graph $\G^{t-}$, which reflects the recent neighborhood structure up to but not including $t$. 

The latent representation for the interaction at time $t$ is then defined as the difference between these two graph perspectives, i.e., 
$
x^t = h^t - h^{t^{-}} 
$,
where $h^t$ and $h^{t^{-}}$ are the graph representations for ego and context graphs, respectively. Here, $h^t$ is computed as
$
h^t = f_o(\text{concat}(z_i^t, z_j^t))
$, where $f_o$ is a two-layer MLP and $z_i^t$ is the outputs of node $i$ for $\G^t$ from the graph encoder. A separate graph encoder with different weights is used to compute $h^{t-}$ for the context graph.

By replacing the original latent representation in the HSC loss with $h^t-h^{t-}$, we formulate the ego-context HSC loss as
\begin{align}
\LL_t^{echsc} =& \ y^t\|h^t - h^{t^{-}}\|^2 - 
  (1-y^t)\log(1-\exp{(-\|h^t - h^{t^{-}}\|^2)})
    \label{eq. ego-context loss}
\end{align}
This modified loss directly measures how an interaction alters the graph representation relative to its historical context, thereby classifying interactions based on their alignment with established patterns in the evolving graph.


\subsubsection{Ego-context Contrastive Loss} 
\label{sec: contrastive loss}

To further prevent overfitting with limited labeled data, we add a contrastive learning component that leverages abundant unlabeled samples. This component maximizes similarity between ego-context graph pairs from the same edge and minimizes similarity between pairs from different edges, based on the assumption that most edges naturally align with their context.

% Here, we aim to harness the rich information in the unlabeled samples, thereby enhancing the ability of the model to discern between normal and anomalous patterns. A straightforward adaptation of the current framework is to maximize the similarity within the ego-context graph pairs from the same edge while minimizing the similarity for pairs from different edges. The underlying assumption is that the majority of edges are aligned with their context, given that the anomalies are rare in real-world situations. 

Specifically, the loss for an edge occurring at time $t$ is defined as:
% \begin{small}
\begin{align}
\LL^{ecc}_t= -\log(S(f_p(h^t), f_p(h^{t^{-}}))) - \log(1-S(f_p(h^t), f_p(h^{t^{-}_{neg}})))
\end{align}
% \end{small}
where $h^{t^{-}_{neg}}$ is the context graph representation of a different edge (selected randomly within a batch), and $S(\cdot, \cdot)$ computes the cosine similarity between two inputs and applies a linear mapping to convert the value within 0 and 1.  The use of $f_p(\cdot)$, an MLP projector function, aligns with standard practices in contrastive learning which ensures that the unsupervised learning framework does not overshadow the primary task. 

Finally, the overall training loss is defined as:
\begin{align}
    \LL = \LL^{echsc} + \lambda \LL^{ecc}
\end{align}
where $\lambda$ is a hyper-parameter controlling the contribution of the contrastive loss. 





==> subtexes/related_works.tex <==








